Optimization Problems for Machine Learning: A Survey

This paper surveys the machine learning literature and presents in an optimization framework several commonly used machine learning approaches. Particularly, mathematical optimization models are presented for regression, classification, clustering, deep learning, and adversarial learning, as well as new emerging applications in machine teaching, empirical model learning, and Bayesian network structure learning. Such models can benefit from the advancement of numerical optimization techniques which have already played a distinctive role in several machine learning settings. The strengths and the shortcomings of these models are discussed and potential research directions and open problems are highlighted.

==> datasets.tex <==
\begin{sidewaystable}[h!]
\setlength{\tabcolsep}{0.03in}
%\begin{table}[h!]
\centering
\begin{tabular}{c|c|c|c|c}
Name &	Description & Size & Default task & Year \\\hline
MNIST &	Handwritten digits & 60,000	& Classification &	1998  \\
CIFAR-10 & Color images & 60,000 & Classification & 2009\\
CIFAR-100 & As CIFAR-10, but 100 classes  & 60,000 & Classification & 2009 \\
ImageNet & Labeled images & 14,197,122  & Object and scene recognition & 2009 \\
ISOLET & Spoken letter names & 7797 & Classification & 1994 \\ 
STL-10 & Color images & 8500 labeled, 10000 unlabeled
 & Classification/Unsupervised learning & 2011 \\ %500 (training) + 8000 (testing); 100000 unlabeled
 \hline
 Higgs & Collision events ($25$ features) & 80,000,000 & Classification & 2015 \\
 Wild & Face images &  $>$13,000 & Classification & 2008\\
 QuocNet & Images & 37,000 & Classification & 2011 \\
 EMNIST & Handwritten characters and digits  & $2,255,710$ ($6$ groups) & Classification & 2017 \\
 Iris & Iris plants & 150 & Classification, pattern recognition & 1936 \\
 Caltech-101 & Images of objects & 9,146 & Classification & 2004 \\
 NORB & Uniform-colored toys & 50 & 3D Object recognition & 2004 \\
 ImageNet Challenge 2012 & Photographs & 150,000 & Visual recognition  & 2012 \\    
Fashion-MNIST & Images & 60,000 & Classification & 2017 \\
SVHN & Digit color images & 630,000 & Classification & 	2011 \\
ACAS dataset & DNN properties & 500 & DNN verification & 2017\\
 CollisionDetection & DNN properties & 188 & DNN verification & 2017\\
 PCAMNIST & DNN properties & 27 & DNN verification & 2018 \\
 TREC Corpus & Messages & 75,419 & Spam classification & 2005 \\
 UCI Spambase Data Set & E-mails & 4,601 & Spam classification & 1999 \\
% Contagio Dataset & Files, multiple formats & 28,760 & Identification of malicious files & 2013\\
 Reuters Corpus & Text documents & 111,740 & Document classification & 2009 \\
 Forest Cover Type & Cartographic variables & 581,012 & Classification & 1999\\ 
 IMDB & Movie reviews & 50,000 & Sentiment classification & 2011\\
 %OR-LIB
 Wine Quality & Wine samples & 4,898 & Classification or regression & 2009 \\
 Wisconsin climatology  & Climate data  &  - & Classification or regression & - \\
 \hline
\end{tabular}
\caption{Datasets - Description.}%
\label{tab:datasets1}
%\end{table}
\end{sidewaystable}
%TODO: Discuss if it makes sense to include datasets for DNN verification. I'd say so.

%\begin{sidewaystable}[h!]
	\begin{table}[h!]
		\begin{minipage}{\textwidth} 
%			\renewcommand\thempfootnote{\arabic{mpfootnote}} % in case I want numbers for the footnote
	\centering
	\begin{tabular}{c|c|c|p{0.3\textwidth}}
		Name & Reference & Repository & Used in \\\hline
		MNIST &	 \cite{lecun1998gradient} & \cite{mnist} & \cite{cheng2017maximum}, \cite{serra2017bounding}, \cite{tjeng2017verifying}, \cite{2017arXiv170207790H}, \cite{bastani2016measuring}, \cite{szegedy2013intriguing}, \cite{good2014}, \cite{carlini2017towards}, \cite{madry2017towards}, \cite{diaz2017effective}, \cite{khalil2018combinatorial}, \cite{fischetti2018deep}, \cite{courbariaux2015binaryconnect}, \cite{globerson2006nightmare}, \cite{dekel2010learning}, \cite{Biggio2013EvasionAA}, \cite{gu2014towards}, \cite{shaham2018understanding}, \cite{rifai2011manifold}, \cite{li2018learning}, \cite{biggio2012poisoning}\\
		CIFAR-10 & \cite{krizhevsky2009learning} & \cite{cifar} & \cite{agos2014}, \cite{bastani2016measuring}, \cite{carlini2017towards}, \cite{madry2017towards}, \cite{courbariaux2015binaryconnect},\cite{good2014}, \cite{shaham2018understanding}, \cite{rifai2011manifold}, \cite{li2018learning}, \cite{SteinhardtKL17}, \cite{lin2013network}, \cite{goodfellow2013maxout}, \cite{WangPoisoning18}, \cite{lin2013network}, \cite{goodfellow2013maxout}\\
		CIFAR-100 & \cite{krizhevsky2009learning} & \cite{cifar} & \cite{agos2014}, \cite{2017arXiv170207790H}, \cite{lin2013network}, \cite{goodfellow2013maxout} \\
		ImageNet & \cite{5206848} & \cite{ImageNet} & \cite{szegedy2013intriguing}, \cite{carlini2017towards}, \cite{kurakin2016adversarial} \\
		ISOLET & \cite{fanty1990spoken} & \cite{Dua2017} & \cite{2017arXiv170207790H}\\ 
		STL-10 & \cite{coates2011analysis} & \cite{STL-10} & \cite{2017arXiv170207790H}\\ %500 (training) + 8000 (testing); 100000 unlabeled
		\hline
		Higgs & \cite{baldi2015enhanced} & Large Hadron Collider & \cite{agos2014} \\
		Wild & \cite{huang2008labeled} & \cite{wild} & \\
%		QuocNet& \cite{le2013building} & Sampled from Wild and ImageNet & \cite{szegedy2013intriguing} \\
		QuocNet& \cite{le2013building} & - & \cite{szegedy2013intriguing} \\
		EMNIST & \cite{Cohen17} & \cite{EMNIST} & - \\
		Iris & \cite{fisher1936use} & \cite{Iris} & - \\
Caltech-101 & \cite{fei2007learning} & \cite{Caltech-101} & \cite{Jarrett2009WhatIT} \\
NORB & \cite{lecun2004learning} & \cite{NORB} & \cite{Jarrett2009WhatIT}\\
ImageNet Challenge 2012 & \cite{ImageNet-Challenge}   & \cite{ILSVRC15} & \cite{he2015delving}\\
		 Fashion-MNIST & \cite{Fashion-MNIST} & \cite{Fashion-MNIST-paper}  & \cite{khalil2018combinatorial}, \cite{WangPoisoning18} \\
		 SVHN & \cite{SVHN} & \cite{netzer2011reading} & \cite{courbariaux2015binaryconnect}, \cite{lin2013network}, \cite{goodfellow2013maxout} \\
ACAS data set & - & \cite{katz2017reluplex} & \cite{katz2017reluplex}, \cite{BunTTKK18}\\
		 CollisionDetection & - & \cite{CollDetect} & \cite{BunTTKK18}\\
		 PCAMNIST & - & \cite{BunTTKK18} & \cite{BunTTKK18} \\
		  TREC Corpus & - & \cite{TREC} & \cite{biggio2010multiple}, \cite{dekel2010learning} \\
		   UCI Spambase Data Set & \cite{UCI} & \cite{UCI-spam} & \cite{dekel2010learning}, \cite{globerson2006nightmare}, \cite{bruckner2012static}, \cite{WangPoisoning18}, \cite{mei2015using} \\
		 %OR-LIB
%		  Contagio Dataset & \cite{UCI} & \cite{UCI-contagio} &  \\
		   Reuters Corpus & \cite{amini2009learning} & \cite{Reuters} & \cite{rifai2011manifold} \\
		   Forest Cover Type & \cite{blackard1999comparative} & \cite{Forest} & \cite{rifai2011manifold}\\
		    IMDB & \cite{maas2011learning} & \cite{IMDB} & \cite{SteinhardtKL17}\\
		  Wine quality & \cite{cortez2009modeling} & \cite{wine} & \cite{mei2015using}\\
 		  Wisconsin climatology  & - &  \cite{madison} & \cite{mei2015using}\footnote{\cite{mei2015using} considered the annual number of frozen days for Lake Mendota in Midwest USA
    		  	from 1900 to 2000. The link provided in their paper is not accessible anymore.}\\ 
		\hline
	\end{tabular}
		\end{minipage}
	\caption{Datasets - References.}
	\label{tab:datasets2}
		\end{table}
%\end{sidewaystable}

%TODO: Dogfish dataset created in https://arxiv.org/pdf/1703.04730.pdf. I don't think it publicly available.
%TODO: Find Contagio in the paper that are citing UCI spam. Probably one is missing.

%TODO: 	  	Spam Bayes filter & \url{http://spambayes.sourceforge.net/} %TODO: Put it into libraries, frameworks   %\cite{barreno2010security} uses it.	  	TREC 2005 & \cite{barreno2010security} & ( 92,189 mails)

%patil2014optimal mentions experiment 2 of another paper. it is not a publicly available dataset.


==> frameworks.tex <==
% !TeX root = ../paper.tex
\begin{sidewaystable}[h!]
%\begin{table}[h!]
	\centering
	\begin{tabular}{c|c|c|c|c}
		Name &	Supported libraries/interfaces  & Purpose & Year & Reference \\\hline
		ConvNetJS &	 Javascript library, online & Training NN &	2014 & \cite{ConvnetJS} \\
		Tensorflow & APIs (Python, Java, C, GO) & Training, evaluating ML/DL models & 2015 & \cite{TF}, \cite{TF-models} \\
		ART & Python library & Adversarial learning & 2017 & \cite{ART-github}, \cite{ART}\\ 
		scikit-learn & Python library & Machine learning & 2011 & \cite{sklearn_api}, \cite{scikit-learn} \\
		Keras & Python library & Deep learning & 2015 & \cite{chollet2015keras} \\
		Theano & Python library & Machine learning & 2016 & \cite{theano}, \cite{2016arXiv160502688short}  \\
		MXNet & APIs (C++, Python, Julia, R, Scala, Perl) & Deep Learning & 2015 & \cite{mxnet}, \cite{mxnet_article} \\
		Pytorch & Python library & Deep learning & 2017 & \cite{pytorch} \\
		Deep Learning for Java & Java APIs & Deep learning & 2014 & \cite{dl4j}\\		
		\hline
	\end{tabular}
	\caption{Frameworks for Machine Learning tasks.}%
	\label{tab:frameworks}
%\end{table}
\end{sidewaystable}


%TODO: the 'Used in' column does not make much of a difference
%TODO: Maybe add Caffe.
%TODO: Double check year of DL4j
%	\begin{tabular}{c|c|c|c|c|c}
%	Name &	Supported libraries/interfaces  & Purpose & Year & Reference  & Used in \\\hline
%	ConvNetJS &	 Javascript library, online & Training NN &	2014 & \cite{ConvnetJS} & \cite{cheng2017maximum}\\
%	Tensorflow & APIs (Python, Java, C, GO) & Training, evaluating ML/DL models & 2015 & \cite{TF}, \cite{TF-models} & \\
%	ART & Python library & Adversarial learning & 2017 & \cite{ART-github}  & \cite{ART}\\ %ART is actually a reference...
%	scikit-learn & Python library & Machine learning & 2011 & \cite{sklearn_api} & \cite{scikit-learn} \\
%	Keras & Python library & Deep learning & 2015 & \cite{chollet2015keras} & \\
%	Theano & Python library & Machine learning & 2016 & \cite{theano} & \cite{2016arXiv160502688short} \\
%	MXNet & APIs (C++, Python, Julia, R, Scala, Perl) & Deep Learning & 2015 & \cite{mxnet} & \cite{mxnet_article}  \\
%	Pytorch & Python library & Deep learning & 2017 & \cite{pytorch} & \\
%	Deep Learning for Java & Java APIs & Deep learning & 2014? & \cite{dl4j} & \cite{Sugomori} \\		
%	\hline
%\end{tabular}




